Multi-dataset Training of Transformers for Robust Action Recognition

We study the task of robust feature representations, aiming to generalize well on multiple datasets for action recognition. We build our method on Transformers for its efficacy. Although we have witnessed great progress for video action recognition in the past decade, it remains challenging yet valuable how to train a single model that can perform well across multiple datasets. Here, we propose a novel multi-dataset training paradigm, MultiTrain, with the design of two new loss terms, namely informative loss and projection loss, aiming to learn robust representations for action recognition. In particular, the informative loss maximizes the expressiveness of the feature embedding while the projection loss for each dataset mines the intrinsic relations between classes across datasets. We verify the effectiveness of our method on five challenging datasets, Kinetics-400, Kinetics-700, Moments-in-Time, Activitynet and Something-something-v2 datasets. Extensive experimental results show that our method can consistently improve state-of-the-art performance. Code and models are released.

==> table/dataset.tex <==
\begingroup
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5} % Default value: 1
\begin{table}
\caption{The number of available videos from Youtube for each split at the time of our experiments compared to the original dataset on release.}
\centering
\begin{tabular}{cccc}
\hline
Dataset      & Train           & Validation     & Released  \\ \hline
Kinetics 400 & 234583 (95.3\%) & 19760 (98.8\%) & May 2017  \\ \hline
Kinetics 700 & 525460 (96.4\%) & 33370 (95.3\%) & July 2019 \\ \hline
\end{tabular}
\label{tab:dataset}
\end{table}
\endgroup

==> table/imgnet.tex <==
\begingroup
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5} % Default value: 1
\begin{table}
\caption{Train from scratch recipe vs. train from ImageNet using MViTv2 16x4 model.}
\centering
\begin{tabular}{c|c}
\hline
Model      & K400 Top-1/5     \\ \hline
MViTv2 16x4 (from scratch 200 ep) &  78.8 / 93.5  \\ \hline
MViTv2 16x4 (from IN-21K-P 75 ep) &  80.6 / 94.7  \\ \hline
\end{tabular}
\label{tab:imgnet}
\end{table}
\endgroup

==> table/projection_all.tex <==
\begingroup
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5} % Default value: 1
\begin{table}
\caption{Visualization of projection weights between different action datasets.
We output the top-5 final cross-dataset projection layer weights of the K400-312p model. 
}
\centering
\resizebox{\columnwidth}{!}{% so there is no overfull
\begin{tabular}{c|c}
\hline
Cross-dataset Pair      & Top-5 Action Pairs   \\ \hline

K400 to MiT &  \begin{tabular}[c]{@{}l@{}} [('bending metal', 'bending'), ('riding elephant', 'skating'), \\ ('pushing wheelchair', 'swinging'), ('tossing coin', 'tattooing'), ('cleaning toilet', 'plunging')]
 \end{tabular}  \\ \hline
 

K400 to SSv2 &  \begin{tabular}[c]{@{}l@{}} [('playing volleyball', 'Covering something with something'),\\ ('washing hair', 'Moving something and something closer to each other'), \\('using computer', 'Pushing something so it spins'), \\('faceplanting', 'Picking something up'), \\('jogging', 'Lifting something with something on it')]
 \end{tabular}  \\ \hline
 
K400 to ActNet &  \begin{tabular}[c]{@{}l@{}} [('parkour', 'Capoeira'), ('running on treadmill', 'Walking the dog'), \\('whistling', 'Snowboarding'), ('water sliding', 'Kayaking'), ('riding mule', 'Canoeing')]
 \end{tabular}  \\ \hline
 
SSv2 to K400 &  \begin{tabular}[c]{@{}l@{}} [('Wiping something off of something', 'cleaning windows'), \\('Throwing something in the air and catching it', 'dining'),\\ ('Pretending or trying and failing to twist something', 'playing poker'), \\('Turning the camera upwards while filming something', 'playing poker'), \\('Pulling two ends of something so that it separates into two pieces', 'dining')]
 \end{tabular}  \\ \hline

SSv2 to MiT &  \begin{tabular}[c]{@{}l@{}} [('Throwing something in the air and catching it', 'hunting'), \\('Turning the camera downwards while filming something', 'flowing'),\\ ('Dropping something into something', 'kneeling'), \\('Pulling two ends of something so that it gets stretched', 'pulling'), \\('Turning the camera upwards while filming something', 'planting')]
 \end{tabular}  \\ \hline

SSv2 to ActNet &  \begin{tabular}[c]{@{}l@{}} [('Turning the camera downwards while filming something', 'Applying sunscreen'), \\('Approaching something with your camera', 'Mooping floor'), \\('Putting something upright on the table', 'Mooping floor'), \\('Turning the camera upwards while filming something', 'Doing fencing'), \\('Showing a photo of something to the camera', 'Playing flauta')]
 \end{tabular}  \\ \hline
 
MiT to K400 &  \begin{tabular}[c]{@{}l@{}} [('gambling', 'bookbinding'), ('autographing', 'eating ice cream'), \\('tearing', 'ripping paper'), ('hitchhiking', 'throwing ball'), ('sneezing', 'sneezing')]
 \end{tabular}  \\ \hline
 
MiT to SSv2 &  \begin{tabular}[c]{@{}l@{}} [('drying', 'Pretending to close something without actually closing it'), \\('twisting', 'Lifting up one end of something without letting it drop down'), \\('fueling', 'Showing something behind something'), \\('trimming', 'Putting something on the edge of something so it is not supported and falls down'), \\('hitchhiking', 'Scooping something up with something')]
 \end{tabular}  \\ \hline

MiT to ActNet &  \begin{tabular}[c]{@{}l@{}} [('fueling', 'Baton twirling'), ('pitching', 'Baton twirling'), \\('snapping', 'Using parallel bars'), ('saluting', 'Baton twirling'), ('frying', 'Waxing skis')]
 \end{tabular}  \\ \hline
 
ActNet to K400 &  \begin{tabular}[c]{@{}l@{}} [('Removing ice from car', 'ski jumping'), ('Playing pool', 'playing badminton'), \\('Hitting a pinata', 'flying kite'), ('Tai chi', 'tai chi'), ('Putting in contact lenses', 'cutting nails')]
 \end{tabular}  \\ \hline

ActNet to MiT &  \begin{tabular}[c]{@{}l@{}} [('Putting on shoes', 'child+singing'), ('Playing piano', 'pushing'), \\('Playing racquetball', 'performing'), ('Washing face', 'drawing'), ('Baton twirling', 'feeding')]
 \end{tabular}  \\ \hline

ActNet to SSv2 &  \begin{tabular}[c]{@{}l@{}} [('Ironing clothes', 'Pretending to be tearing something that is not tearable'), \\('Tai chi', 'Throwing something'),\\ ('Doing step aerobics', 'Pushing something so that it falls off the table'), \\('Doing crunches', 'Pushing something so that it slightly moves'), \\('Getting a tattoo', "Tilting something with something on it slightly so it doesn't fall down")]

 \end{tabular}  \\ \hline
 
\end{tabular}
}
\label{tab:proj_all}
\end{table}
\endgroup
